Warm-Start Variational Quantum Policy Iteration

Reinforcement learning is a powerful framework aiming to determine optimal behavior in highly complex decision-making scenarios. This objective can be achieved using policy iteration, which requires to solve a typically large linear system of equations. We propose the variational quantum policy iteration (VarQPI) algorithm, realizing this step with a NISQ-compatible quantum-enhanced subroutine. Its scalability is supported by an analysis of the structure of generic reinforcement learning environments, laying the foundation for potential quantum advantage with utility-scale quantum computers. Furthermore, we introduce the warm-start initialization variant (WS-VarQPI) that significantly reduces resource overhead. The algorithm solves a large FrozenLake environment with an underlying 256x256-dimensional linear system, indicating its practical robustness.

==> figures/resources.tex <==
\begin{figure*}[t]
    \usetikzlibrary{calc}
    \centering
    \begin{minipage}{0.69\linewidth}
        \subfigure[aa]{
            \begin{tikzpicture}
                \begin{axis}[
                    name=plot2,
                    % xlabel=$\textbf{qubits}$,
                    ylabel=$\textbf{success rate}$,
                    xmode=log,
                    xtick={0.00002, 0.00005, 0.0001, 0.0002, 0.0005, 0.001, 0.002, 0.005, 0.01, 0.02, 0.05},
                    xticklabels={},
                    ytick={0.25, 0.5, 0.75, 1.0},
                    yticklabels={$25\%$,$50\%$,$75\%$,$100\%$},
                    xmin=0.000016,xmax=0.065,
                    ymin=0.20,ymax=1.1,
                    label style={font=\footnotesize},
                    tick label style={font=\footnotesize},
                    grid=both,
                    axis x line=bottom, axis y line=left,
                    width=0.99\linewidth,
                    height=4cm,
                    legend style={/tikz/every even column/.append style={column sep=0.1cm, row sep=0.1cm},at={(0.3,0.6)},anchor=east,yshift=-5mm,font=\scriptsize}]
                    ]
        
                    % perturbation 0.0
                    \addplot[line width=.7pt,solid,color=col_per00,mark=o] %
                    	table[x=threshold,y=per0.0,col sep=comma]{figures/data/threshold.csv};
        
                    % perturbation 0.1
                    \addplot[line width=.7pt,solid,color=col_per01,mark=o] %
                    	table[x=threshold,y=per0.1,col sep=comma]{figures/data/threshold.csv};
        
                    % perturbation 0.3
                    \addplot[line width=.7pt,solid,color=col_per03,mark=o] %
                    	table[x=threshold,y=per0.3,col sep=comma]{figures/data/threshold.csv};
        
                    \legend{$\beta=0.0$,$\beta=0.1$,$\beta=0.3$};
        
                    % \addplot [mark=none, black] {0.95};
                \end{axis}
            \end{tikzpicture}
        }
    \end{minipage}
    \begin{minipage}{0.29\linewidth}
        \subfigure[aa]{
            \includegraphics[width=\textwidth]{figures/env_large.pdf}
        }
    \end{minipage}
        \subfigure[aa]{
            \begin{tikzpicture}
                \begin{axis}[
                    name=plot2,
                    % xlabel=$\textbf{qubits}$,
                    ylabel=$\textbf{success rate}$,
                    xmode=log,
                    xtick={0.00002, 0.00005, 0.0001, 0.0002, 0.0005, 0.001, 0.002, 0.005, 0.01, 0.02, 0.05},
                    xticklabels={},
                    ytick={0.25, 0.5, 0.75, 1.0},
                    yticklabels={$25\%$,$50\%$,$75\%$,$100\%$},
                    xmin=0.000016,xmax=0.065,
                    ymin=0.20,ymax=1.1,
                    label style={font=\footnotesize},
                    tick label style={font=\footnotesize},
                    grid=both,
                    axis x line=bottom, axis y line=left,
                    width=0.99\linewidth,
                    height=4cm,
                    legend style={/tikz/every even column/.append style={column sep=0.1cm, row sep=0.1cm},at={(0.3,0.6)},anchor=east,yshift=-5mm,font=\scriptsize}]
                    ]
        
                    % perturbation 0.0
                    \addplot[line width=.7pt,solid,color=col_per00,mark=o] %
                    	table[x=threshold,y=per0.0,col sep=comma]{figures/data/threshold.csv};
        
                    % perturbation 0.1
                    \addplot[line width=.7pt,solid,color=col_per01,mark=o] %
                    	table[x=threshold,y=per0.1,col sep=comma]{figures/data/threshold.csv};
        
                    % perturbation 0.3
                    \addplot[line width=.7pt,solid,color=col_per03,mark=o] %
                    	table[x=threshold,y=per0.3,col sep=comma]{figures/data/threshold.csv};
        
                    \legend{$\beta=0.0$,$\beta=0.1$,$\beta=0.3$};
        
                    % \addplot [mark=none, black] {0.95};
        
                \end{axis}
                \begin{axis}[
                    name=plot3,
                    at={($(plot2.south)+(0,-0.5cm)$)}, anchor=north,
                    xlabel=$\textbf{loss threshold}$,
                    xlabel shift=18pt,
                    ylabel=$\textbf{steps}$,
                    % xmode=log,
                    % ymode=log,
                    % xtick={0.00002, 0.00005, 0.0001, 0.0002, 0.0005, 0.001, 0.002, 0.005, 0.01, 0.02, 0.05},
                    % xticklabels={$2$, $5$, $1$, $2$, $5$, $1$, $2$, $5$, $1$, $2$, $5$},
                    ytick={0, 50, 100},
                    % yticklabels={$0$,$1500$, $3000$},
                    xmin=1.0,xmax=14.0,
                    ymin=0.0,ymax=100.0,
                    % restrict y to domain=-2000:3100;
                    clip=false,
                    label style={font=\footnotesize},
                    tick label style={font=\footnotesize},
                    grid=both,
                    axis x line=bottom, axis y line=left,
                    width=0.99\linewidth,
                    height=4cm,
                    legend style={/tikz/every even column/.append style={column sep=0.1cm, row sep=0.1cm},at={(0.33,0.88)},anchor=east,yshift=-5mm,font=\scriptsize}]
                    ]
        
                    % size 4
                    \addplot[line width=.7pt,solid,color=col_per00,mark=o] %
                    	table[x=depth,y=converged,col sep=comma]{figures/data/ChainWalk_size=4.csv};

                    % size 8
                    \addplot[line width=.7pt,solid,color=col_per00,mark=o] %
                    	table[x=depth,y=converged,col sep=comma]{figures/data/ChainWalk_size=8.csv};

                    % size 16
                    \addplot[line width=.7pt,solid,color=col_per00,mark=o] %
                    	table[x=depth,y=converged,col sep=comma]{figures/data/ChainWalk_size=16.csv};

                    % size 16
                    \addplot[line width=.7pt,solid,color=col_per00,mark=o] %
                    	table[x=depth,y=converged,col sep=comma]{figures/data/ChainWalk_size=32.csv};

                                        % size 16
                    \addplot[line width=.7pt,solid,color=col_per00,mark=o] %
                    	table[x=depth,y=converged,col sep=comma]{figures/data/ChainWalk_size=64.csv};
        
                \end{axis}   
            \end{tikzpicture}
        }
    \caption{\label{fig:resources}Success rates of variational quantum policy evaluation for different loss thresholds and therefore required training steps. The results are averaged over $1000$ random instances of \texttt{FrozenLake} with varying stochasticity $\beta$. Training is terminated once the loss value $C_{G}$ has declined below the given threshold. The success rate denotes the percentage of runs for which \cref{eq:greedy_action_selection} agrees with the ground truth. To account for sampling noise, we tolerate a deviation of $0.001$ in the associated $Q$-values.}
\end{figure*}
